Dependency Parsing with Backtracking using Deep Reinforcement Learning

Greedy algorithms for NLP such as transition based parsing are prone to error propagation. One way to overcome this problem is to allow the algorithm to backtrack and explore an alternative solution in cases where new evidence contradicts the solution explored so far. In order to implement such a behavior, we use reinforcement learning and let the algorithm backtrack in cases where such an action gets a better reward than continuing to explore the current solution. We test this idea on both POS tagging and dependency parsing and show that backtracking is an effective means to fight against error propagation.

==> figures/allStats.tex <==
\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{PARSER} \\ \hline
\texttt{\#Actions} & \texttt{82,552} \\ \hline
\texttt{\#Errs} & \texttt{4,122} \\ \hline
\texttt{\#Backs} & \texttt{1,134} \\ \hline
\texttt{bPrec} & \texttt{72.31\%} \\ \hline
\texttt{bRec} & \texttt{22.10\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{22.46\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{50.53\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{05.26\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{21.75\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Arabic-PADT eager}
\label{tab:Stats for rlb in Arabic-PADT eager}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAGGER} \\ \hline
\texttt{\#Actions} & \texttt{56,528} \\ \hline
\texttt{\#Errs} & \texttt{1,093} \\ \hline
\texttt{\#Backs} & \texttt{310} \\ \hline
\texttt{bPrec} & \texttt{58.06\%} \\ \hline
\texttt{bRec} & \texttt{16.47\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{39.35\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{29.03\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{02.58\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{29.03\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Arabic-PADT tagger}
\label{tab:Stats for rlb in Arabic-PADT tagger}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAPARSER} \\ \hline
\texttt{\#Actions} & \texttt{110,150} \\ \hline
\texttt{\#Errs} & \texttt{5,896} \\ \hline
\texttt{\#Backs} & \texttt{3,145} \\ \hline
\texttt{bPrec} & \texttt{67.15\%} \\ \hline
\texttt{bRec} & \texttt{42.57\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{59.98\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{27.34\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{02.98\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{09.70\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Arabic-PADT tagparser}
\label{tab:Stats for rlb in Arabic-PADT tagparser}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{PARSER} \\ \hline
\texttt{\#Actions} & \texttt{33,939} \\ \hline
\texttt{\#Errs} & \texttt{3,444} \\ \hline
\texttt{\#Backs} & \texttt{2,309} \\ \hline
\texttt{bPrec} & \texttt{79.30\%} \\ \hline
\texttt{bRec} & \texttt{59.87\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{15.68\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{43.58\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{05.21\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{35.53\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Chinese-GSD eager}
\label{tab:Stats for rlb in Chinese-GSD eager}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAGGER} \\ \hline
\texttt{\#Actions} & \texttt{24,024} \\ \hline
\texttt{\#Errs} & \texttt{933} \\ \hline
\texttt{\#Backs} & \texttt{318} \\ \hline
\texttt{bPrec} & \texttt{68.55\%} \\ \hline
\texttt{bRec} & \texttt{23.37\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{29.56\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{37.42\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{01.89\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{31.13\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Chinese-GSD tagger}
\label{tab:Stats for rlb in Chinese-GSD tagger}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAPARSER} \\ \hline
\texttt{\#Actions} & \texttt{45,603} \\ \hline
\texttt{\#Errs} & \texttt{4,884} \\ \hline
\texttt{\#Backs} & \texttt{3,940} \\ \hline
\texttt{bPrec} & \texttt{75.66\%} \\ \hline
\texttt{bRec} & \texttt{74.10\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{55.41\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{27.70\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{02.81\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{14.09\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Chinese-GSD tagparser}
\label{tab:Stats for rlb in Chinese-GSD tagparser}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{PARSER} \\ \hline
\texttt{\#Actions} & \texttt{45,696} \\ \hline
\texttt{\#Errs} & \texttt{3,845} \\ \hline
\texttt{\#Backs} & \texttt{2,248} \\ \hline
\texttt{bPrec} & \texttt{81.72\%} \\ \hline
\texttt{bRec} & \texttt{62.68\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{12.14\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{35.71\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{06.25\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{45.90\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in English-GUM eager}
\label{tab:Stats for rlb in English-GUM eager}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAGGER} \\ \hline
\texttt{\#Actions} & \texttt{31,852} \\ \hline
\texttt{\#Errs} & \texttt{1,097} \\ \hline
\texttt{\#Backs} & \texttt{691} \\ \hline
\texttt{bPrec} & \texttt{72.94\%} \\ \hline
\texttt{bRec} & \texttt{45.94\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{24.31\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{27.06\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{02.75\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{45.88\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in English-GUM tagger}
\label{tab:Stats for rlb in English-GUM tagger}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAPARSER} \\ \hline
\texttt{\#Actions} & \texttt{60,750} \\ \hline
\texttt{\#Errs} & \texttt{5,480} \\ \hline
\texttt{\#Backs} & \texttt{4,216} \\ \hline
\texttt{bPrec} & \texttt{75.90\%} \\ \hline
\texttt{bRec} & \texttt{76.15\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{55.98\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{25.42\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{02.63\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{15.97\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in English-GUM tagparser}
\label{tab:Stats for rlb in English-GUM tagparser}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{PARSER} \\ \hline
\texttt{\#Actions} & \texttt{29,018} \\ \hline
\texttt{\#Errs} & \texttt{1,105} \\ \hline
\texttt{\#Backs} & \texttt{436} \\ \hline
\texttt{bPrec} & \texttt{74.31\%} \\ \hline
\texttt{bRec} & \texttt{31.95\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{20.18\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{41.06\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{05.50\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{33.26\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in French-GSD eager}
\label{tab:Stats for rlb in French-GSD eager}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAGGER} \\ \hline
\texttt{\#Actions} & \texttt{20,038} \\ \hline
\texttt{\#Errs} & \texttt{350} \\ \hline
\texttt{\#Backs} & \texttt{252} \\ \hline
\texttt{bPrec} & \texttt{66.67\%} \\ \hline
\texttt{bRec} & \texttt{48.00\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{30.16\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{23.02\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{03.17\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{43.65\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in French-GSD tagger}
\label{tab:Stats for rlb in French-GSD tagger}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAPARSER} \\ \hline
\texttt{\#Actions} & \texttt{38,771} \\ \hline
\texttt{\#Errs} & \texttt{1,815} \\ \hline
\texttt{\#Backs} & \texttt{1,159} \\ \hline
\texttt{bPrec} & \texttt{71.79\%} \\ \hline
\texttt{bRec} & \texttt{55.10\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{57.31\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{25.55\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{02.83\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{14.32\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in French-GSD tagparser}
\label{tab:Stats for rlb in French-GSD tagparser}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{PARSER} \\ \hline
\texttt{\#Actions} & \texttt{935,414} \\ \hline
\texttt{\#Errs} & \texttt{22,829} \\ \hline
\texttt{\#Backs} & \texttt{11,970} \\ \hline
\texttt{bPrec} & \texttt{71.88\%} \\ \hline
\texttt{bRec} & \texttt{43.83\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{21.88\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{30.46\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{06.20\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{41.46\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in German-HDT eager}
\label{tab:Stats for rlb in German-HDT eager}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAGGER} \\ \hline
\texttt{\#Actions} & \texttt{652,500} \\ \hline
\texttt{\#Errs} & \texttt{54,173} \\ \hline
\texttt{\#Backs} & \texttt{53,573} \\ \hline
\texttt{bPrec} & \texttt{95.88\%} \\ \hline
\texttt{bRec} & \texttt{94.83\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{03.77\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{07.35\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{00.35\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{88.53\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in German-HDT tagger}
\label{tab:Stats for rlb in German-HDT tagger}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAPARSER} \\ \hline
\texttt{\#Actions} & \texttt{1,255,003} \\ \hline
\texttt{\#Errs} & \texttt{45,206} \\ \hline
\texttt{\#Backs} & \texttt{32,748} \\ \hline
\texttt{bPrec} & \texttt{68.80\%} \\ \hline
\texttt{bRec} & \texttt{60.45\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{59.90\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{18.83\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{03.19\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{18.08\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in German-HDT tagparser}
\label{tab:Stats for rlb in German-HDT tagparser}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{PARSER} \\ \hline
\texttt{\#Actions} & \texttt{47,179} \\ \hline
\texttt{\#Errs} & \texttt{2,146} \\ \hline
\texttt{\#Backs} & \texttt{723} \\ \hline
\texttt{bPrec} & \texttt{70.68\%} \\ \hline
\texttt{bRec} & \texttt{25.86\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{24.79\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{41.32\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{04.41\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{29.48\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Romanian-RRT eager}
\label{tab:Stats for rlb in Romanian-RRT eager}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAGGER} \\ \hline
\texttt{\#Actions} & \texttt{32,648} \\ \hline
\texttt{\#Errs} & \texttt{605} \\ \hline
\texttt{\#Backs} & \texttt{330} \\ \hline
\texttt{bPrec} & \texttt{66.06\%} \\ \hline
\texttt{bRec} & \texttt{36.03\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{30.61\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{24.55\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{03.33\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{41.52\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Romanian-RRT tagger}
\label{tab:Stats for rlb in Romanian-RRT tagger}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAPARSER} \\ \hline
\texttt{\#Actions} & \texttt{63,141} \\ \hline
\texttt{\#Errs} & \texttt{3,234} \\ \hline
\texttt{\#Backs} & \texttt{2,204} \\ \hline
\texttt{bPrec} & \texttt{66.74\%} \\ \hline
\texttt{bRec} & \texttt{55.53\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{59.82\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{25.04\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{03.24\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{11.89\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Romanian-RRT tagparser}
\label{tab:Stats for rlb in Romanian-RRT tagparser}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{PARSER} \\ \hline
\texttt{\#Actions} & \texttt{335,580} \\ \hline
\texttt{\#Errs} & \texttt{14,175} \\ \hline
\texttt{\#Backs} & \texttt{6,129} \\ \hline
\texttt{bPrec} & \texttt{74.01\%} \\ \hline
\texttt{bRec} & \texttt{34.74\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{19.88\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{40.32\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{06.21\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{33.59\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Russian-SynTagRus eager}
\label{tab:Stats for rlb in Russian-SynTagRus eager}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAGGER} \\ \hline
\texttt{\#Actions} & \texttt{234,658} \\ \hline
\texttt{\#Errs} & \texttt{19,374} \\ \hline
\texttt{\#Backs} & \texttt{19,435} \\ \hline
\texttt{bPrec} & \texttt{95.64\%} \\ \hline
\texttt{bRec} & \texttt{95.94\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{04.21\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{05.40\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{00.16\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{90.23\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Russian-SynTagRus tagger}
\label{tab:Stats for rlb in Russian-SynTagRus tagger}
\end{table}

\begin{table}[htbp]
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|}
\hline
 & \textbf{TAPARSER} \\ \hline
\texttt{\#Actions} & \texttt{449,118} \\ \hline
\texttt{\#Errs} & \texttt{20,566} \\ \hline
\texttt{\#Backs} & \texttt{16,734} \\ \hline
\texttt{bPrec} & \texttt{67.40\%} \\ \hline
\texttt{bRec} & \texttt{62.67\%} \\ \hline
\texttt{C$\rightarrow$C} & \texttt{61.57\%} \\ \hline
\texttt{E$\rightarrow$E} & \texttt{19.94\%} \\ \hline
\texttt{C$\rightarrow$E} & \texttt{03.34\%} \\ \hline
\texttt{E$\rightarrow$C} & \texttt{15.14\%} \\ \hline
\end{tabular}
\caption{Stats for rlb in Russian-SynTagRus tagparser}
\label{tab:Stats for rlb in Russian-SynTagRus tagparser}
\end{table}


==> figures/parser_all_stats.tex <==
\begin{table}[]
\tabcolsep=0.8mm
\begin{tabular}{lrrrrrrr}
\texttt{Lang}	& \textbf{FR} 	& \textbf{EN} 	& \textbf{DE} 	& \textbf{RO} 	& \textbf{RU} 	& \textbf{AR} 	& \textbf{ZH} \\
\texttt{\#Act}	& \texttt{29,018} 	& \texttt{45,696} 	& \texttt{935,414} 	& \texttt{47,179} 	& \texttt{335,580} 	& \texttt{82,552} 	& \texttt{33,939} \\
\texttt{\#Errs} 	& \texttt{1,105} 	& \texttt{3,845} 	& \texttt{22,829} 	& \texttt{2,146} 	& \texttt{14,175} 	& \texttt{4,122} 	& \texttt{3,444} \\
\texttt{\#Backs} 	& \texttt{436} 	& \texttt{2,248} 	& \texttt{11,970} 	& \texttt{723} 	& \texttt{6,129} 	& \texttt{1,134} 	& \texttt{2,309} \\
\texttt{bPrec} 	& \texttt{74.31\%} 	& \texttt{81.72\%} 	& \texttt{71.88\%} 	& \texttt{70.68\%} 	& \texttt{74.01\%} 	& \texttt{72.31\%} 	& \texttt{79.30\%} \\
\texttt{bRec} 	& \texttt{31.95\%} 	& \texttt{62.68\%} 	& \texttt{43.83\%} 	& \texttt{25.86\%} 	& \texttt{34.74\%} 	& \texttt{22.10\%} 	& \texttt{59.87\%} \\
\texttt{C$\rightarrow$C} 	& \texttt{20.18\%} 	& \texttt{12.14\%} 	& \texttt{21.88\%} 	& \texttt{24.79\%} 	& \texttt{19.88\%} 	& \texttt{22.46\%} 	& \texttt{15.68\%} \\
\texttt{E$\rightarrow$E} 	& \texttt{41.06\%} 	& \texttt{35.71\%} 	& \texttt{30.46\%} 	& \texttt{41.32\%} 	& \texttt{40.32\%} 	& \texttt{50.53\%} 	& \texttt{43.58\%} \\
\texttt{C$\rightarrow$E} 	& \texttt{05.50\%} 	& \texttt{06.25\%} 	& \texttt{06.20\%} 	& \texttt{04.41\%} 	& \texttt{06.21\%} 	& \texttt{05.26\%} 	& \texttt{05.21\%} \\
\texttt{E$\rightarrow$C} 	& \texttt{33.26\%} 	& \texttt{45.90\%} 	& \texttt{41.46\%} 	& \texttt{29.48\%} 	& \texttt{33.59\%} 	& \texttt{21.75\%} 	& \texttt{35.53\%} \\
\end{tabular}	
\caption{Parser}
\label{tab:stats_parser_multi}
\end{table}

==> figures/resGPS.tex <==
\begin{table}
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{UAS} & \textbf{p} \\ \hline
SL & 88.38 & 0.421 \\ \hline
RL\_BT1 & 87.50 & 0.421 \\ \hline
RL\_NOBT & 86.56 & \_ \\ \hline
\end{tabular}
\caption{eager on Garden Path Sentences}
\label{tab:res_eager}
\end{table}


\begin{table}
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{UPOS} & \textbf{p} \\ \hline
RL\_BT1 & 84.29 & 0.050 \\ \hline
RL\_NOBT & 79.06 & 0.352 \\ \hline
SL & 77.78 & \_ \\ \hline
\end{tabular}
\caption{tagger on Garden Path Sentences}
\label{tab:res_tagger}
\end{table}


\begin{table}
\centering
\tabcolsep=0.8mm
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{UAS} & \textbf{p} & \textbf{UPOS} & \textbf{p} \\ \hline
RL\_BT1 & 86.79 & 0.406 & 79.31 & 0.334 \\ \hline
RL\_NOBT & 85.94 & 0.128 & 79.65 & 0.458 \\ \hline
SL & 81.25 & \_ & 78.09 & \_ \\ \hline
\end{tabular}
\caption{tagparser on Garden Path Sentences}
\label{tab:res_tagparser}
\end{table}


==> figures/resMultilingBackup.tex <==
\begin{table}[htb]
\tabcolsep=0.8mm
\centering
\begin{tabular}{@{}lrrrr@{}} \toprule
& TAGGER & PARSER & \multicolumn{2}{c}{TAGPARSER} \\
Regime & UPOS & UAS & UPOS & UAS \\ \midrule
\multicolumn{5}{c}{French} \\
\rlbt{} & \bf{97.52} & \bf{87.69} & \bf{96.49} & \bf{84.51} \\
\rl{} & 96.64 & 86.63 & 96.01 & 83.68 \\
\sul{} & 96.25 & 86.96 & 96.35 & 83.69 \\
\multicolumn{5}{c}{English} \\
\rlbt{} & \bf{94.98} & \bf{79.95} & \bf{93.95} & \bf{74.12} \\
\rl{} & 93.53 & 72.97 & 93.20 & 69.93 \\
\sul{} & 92.63 & 73.12 & 93.09 & 69.84 \\
\multicolumn{5}{c}{German} \\
\rlbt{} & \bf{97.88} & \bf{92.89} & \bf{97.21} & \bf{90.01} \\
\rl{} & 97.29 & 91.25 & 96.99 & 89.66 \\
\sul{} & 97.28 & 91.19 & 97.16 & 89.44 \\
\multicolumn{5}{c}{Romanian} \\
\rlbt{} & \bf{97.07} & \bf{85.40} & \bf{95.96} & \bf{83.43} \\
\rl{} & 96.28 & 84.70 & 95.84 & 82.54 \\
\sul{} & 95.77 & 84.99 & 95.83 & 82.87 \\
\multicolumn{5}{c}{Russian} \\
\rlbt{} & \bf{98.41} & \bf{86.59} & \bf{97.77} & \bf{84.52} \\
\rl{} & 97.93 & 85.25 & 97.59 & 83.86 \\
\sul{} & 97.80 & 85.28 & 97.73 & 83.88 \\
\multicolumn{5}{c}{Arabic} \\
\rlbt{} & \bf{96.42} & 83.81 & 95.55 & 82.50 \\
\rl{} & 96.20 & 83.76 & \bf{95.92} & 82.48 \\
\sul{} & 95.73 & \bf{83.94} & 95.89 & \bf{82.84} \\
\multicolumn{5}{c}{Chinese} \\
\rlbt{} & \bf{93.01} & \bf{71.69} & 91.56 & \bf{65.68} \\
\rl{} & 91.61 & 64.63 & 91.53 & 60.07 \\
\sul{} & 91.30 & 65.78 & \bf{91.63} & 61.79 \\
\bottomrule
\end{tabular}
\caption{Results for seven languages.}
\label{tab:resMultiling}
\end{table}


==> figures/tagger_all_stats.tex <==
\begin{table}[]
\tabcolsep=0.8mm
\begin{tabular}{lrrrrrrr}
\texttt{Lang}	& \textbf{FR} &	\textbf{EN} &	\textbf{DE} &	\textbf{RO} &	\textbf{RU} &	\textbf{AR} &	\textbf{ZH}	\\
\texttt{\#Act}	&\texttt{20,038} &	\texttt{31,852} &	\texttt{652,500} &	\texttt{32,648} &	\texttt{234,658} &	\texttt{56,528} &	\texttt{24,024}	\\
\texttt{\#Errs}	&\texttt{350} &	\texttt{1,097} &	\texttt{54,173} &	\texttt{605} &	\texttt{19,374} &	\texttt{1,093} &	\texttt{933}	\\
\texttt{\#Backs} &	\texttt{252} &	\texttt{691} &	\texttt{53,573} &	\texttt{330} &	\texttt{19,435} &	\texttt{310} &	\texttt{318}	\\
\texttt{bPrec} &	\texttt{66.67\%} &	\texttt{72.94\%} &	\texttt{95.88\%} &	\texttt{66.06\%} &	\texttt{95.64\%} &	\texttt{58.06\%} &	\texttt{68.55\%}	\\
\texttt{bRec} &	\texttt{48.00\%} &	\texttt{45.94\%} &	\texttt{94.83\%} &	\texttt{36.03\%} &	\texttt{95.94\%} &	\texttt{16.47\%} &	\texttt{23.37\%}	\\
\texttt{C$\rightarrow$C} &	\texttt{30.16\%} &	\texttt{24.31\%} &	\texttt{03.77\%} &	\texttt{30.61\%} &	\texttt{04.21\%} &	\texttt{39.35\%} &	\texttt{29.56\%}	\\
\texttt{E$\rightarrow$E} &	\texttt{23.02\%} &	\texttt{27.06\%} &	\texttt{07.35\%} &	\texttt{24.55\%} &	\texttt{05.40\%} &	\texttt{29.03\%} &	\texttt{37.42\%}	\\
\texttt{C$\rightarrow$E} &	\texttt{03.17\%} &	\texttt{02.75\%} &	\texttt{00.35\%} &	\texttt{03.33\%} &	\texttt{00.16\%} &	\texttt{02.58\%} &	\texttt{01.89\%}	\\
\texttt{E$\rightarrow$C} &	\texttt{43.65\%} &	\texttt{45.88\%} &	\texttt{88.53\%} &	\texttt{41.52\%} &	\texttt{90.23\%} &	\texttt{29.03\%} &	\texttt{31.13\%}	\\
\end{tabular}
\caption{Tagger}
\label{tab:stats_tagger_multi}
\end{table}
